High Probability Bound for Cross-Learning Contextual Bandits with Unknown Context Distributions

Motivated by applications in online bidding and sleeping bandits, we examine the problem of contextual bandits with cross learning, where the learner observes the loss associated with the action across all possible contexts, not just the current round's context. Our focus is on a setting where losses are chosen adversarially, and contexts are sampled i.i.d. from a specific distribution. This problem was first studied by Balseiro et al. (2019), who proposed an algorithm that achieves near-optimal regret under the assumption that the context distribution is known in advance. However, this assumption is often unrealistic. To address this issue, Schneider and Zimmert (2023) recently proposed a new algorithm that achieves nearly optimal expected regret. It is well-known that expected regret can be significantly weaker than high-probability bounds. In this paper, we present a novel, in-depth analysis of their algorithm and demonstrate that it actually achieves near-optimal regret with high probability. There are steps in the original analysis by Schneider and Zimmert (2023) that lead only to an expected bound by nature. In our analysis, we introduce several new insights. Specifically, we make extensive use of the weak dependency structure between different epochs, which was overlooked in previous analyses. Additionally, standard martingale inequalities are not directly applicable, so we refine martingale inequalities to complete our analysis.

==> high_probability.tex <==
\section{High Probability Bound of [Zimmert 2023]}

%假设我们单独有一章，介绍过 Zimmert 2023 的算法。
%假设我们曾经解释 F_e L_e G 是什么意思
%假设解释了 p_t(a) 的意思

%\subsection{New Analysis}
In this section we improve the expected regret bound in [Zimmert 2023] to a high probability regret bound. 

Fix a policy $\pi : [C] \rightarrow [K]$. With a slight abuse of notation, we also denote $\pi_c = e_k \in \Delta([K])$ for each $c \in [C]$. The (unexpected) regret with respect to policy $\pi$ is
\[\Reg(\pi) = \sum_{t=1}^T \ell_{t, c_t}(a_t) -  \ell_{t, c_t}(\pi_{c_t}) .\]
We would like to upper bound this quantity (for an arbitrary $\pi$).

We will prove the following result.
\begin{theorem}
\label{thm:high_probability_main}
    For $\iota=2 \log (8 K T)$, $L=\sqrt{\frac{\iota K T}{\log (K)}}=\widetilde{\Theta}(\sqrt{K T})$, $\gamma=\frac{16 \iota}{L}=\widetilde{\Theta}(1 / \sqrt{K T})$, and $\eta=\frac{\gamma}{2(2 L \gamma+\iota)}=\widetilde{\Theta}(1 / \sqrt{K T})$, \Cref{alg:main}  yields a regret bound of $\Reg(\pi)= \widetilde{\Theta}(\sqrt{KT})$ with high probability.
\end{theorem}

[Zimmert 2023] showed that \Cref{alg:main} yields an expected regret bound of $\E[\Reg(\pi)]  = \widetilde{\Theta}(\sqrt{KT})$. Our theorem extends this result. We show that the exact same algorithm actually yields a high probability regret bound.

Here we explain the key observation behind \cref{thm:high_probability_main}. To explain our observation, we need to first explain why the analysis in [Zimmert 2023] cannot give a high probability bound.
%first. 
The main problem is that the analysis in [Zimmert 2023] cannot give a small enough bound for the bias of the estimator of the inverse importance weighting factor $\frac{1}{f_{ek}} - \frac{1}{\widehat{f}_{ek}}$. 
%
[Zimmert 2023] only uses samples come from epoch $e-1$ to construct the estimator $\frac{1}{\widehat{f}_{ek}}$ because they need to ensure these samples are mutually independent.
%
Thus the estimator  $\frac{1}{\widehat{f}_{ek}}$ is constructed  from a limited number of samples and the bias $\frac{1}{f_{ek}} - \frac{1}{\widehat{f}_{ek}}$ is too large.
%
To get small enough bias with a limited sample number, [Zimmert 2023] only bound the expected bias $\E[\frac{1}{f_{ek}} - \frac{1}{\widehat{f}_{ek}}]$. Thus they only bound the expected regret and cannot give a high probability regret bound.
%
% After introducing the key technique used in [Zimmert 2023], we can state our key observation behind \cref{thm:high_probability_main}. 
In contrast, we note that different epochs in \Cref{alg:main}  are only weakly dependent from each other.
%
Thus, the bias $\frac{1}{f_{ek}} - \frac{1}{\widehat{f}_{ek}}$ of each epoch $e$ is also only weakly dependent from each other.
%
Thus, although we cannot give a small enough bound for the bias of one epoch $\frac{1}{f_{ek}} - \frac{1}{\widehat{f}_{ek}}$, we can give a small enough bound for the cumulative bias of all epochs $\sum_e \frac{1}{f_{ek}} - \frac{1}{\widehat{f}_{ek}}$. And we use the bound on cumulative bias to bound the cumulative regret.

We now dive into our argument for upper bounding the unexpected regret. 

We firstly establish a reduction. 
%
In [Zimmert 2023], \Cref{alg:main} groups all time steps into consecutive pairs. In each pair of consecutive time steps, the algorithm plays the same distribution and randomly uses one to calculate a loss estimate, and the other to estimate the sampling frequency. 
%
We show that it is enough to have a high probability regret bound only on the loss sequence used in calculating loss estimates. This reduction is crucial for establishing the weak dependence structure between different epochs, which is crucial for our result.


\begin{lemma}
\label{lemma:used_loss_reduction}
 Decomposing all time steps into consecutive pairs, i.e. decomposing $\{1,2,\dots,T\}$ into $\{ (1,2), (3,4), (5,6), \dots, (t-1,t), \dots, (T-1,T)\}$.
 %
 Constructing a surrogate loss sequence $\{\widetilde{\ell}_s\}_{s=1}^{\frac{T}{2}}$ such that for each surrogate time step $s$ the loss vector $\widetilde{\ell}_s$ for each $s$ is uniformly sampled from the pair of true loss vector $(\ell_{2s-1},\ell_{2s})$.  Denote the time step sampled from the pair $(2s-1,2s)$ as $s_{\ell}$. 
 %
 For any constant $\delta \in (0,1)$ and any bandit algorithm such that in each pair of time steps $(t-1,t)$, the algorithm takes action $a_{t-1}$ and $a_t$ from the same distribution $p_{t-1} = p_t$, we have
\[ \sum_{t=1}^T \left( \ell_{t, c_t}(a_t) -  \ell_{t, c_t}(\pi_{c_t}) \right) \le 2 \sum_{s=1}^{\frac{T}{2}} \left( \widetilde{\ell}_{s,c_{s_{\ell}}}(a_{s_{\ell}}) - \widetilde{\ell}_{s,c_{s_{\ell}}}(\pi_{c_{s_{\ell}}}) \right) + 2 \sqrt{T \log(\frac{1}{\delta})} \]
with probability at least $1 - \delta$.
%
\end{lemma}

This lemma shows that we only need to get a high probability regret bound on the surrogate loss sequence $\widetilde{\ell}_s$. Applying \cref{lemma:used_loss_reduction} on \Cref{alg:main}, we get that we only need to upper bound the regret on the loss sequence used in calculating loss estimates. 

\begin{proof}[Proof of \cref{lemma:used_loss_reduction}]
    Consider the sequence of random variable $\{Y_s\}_{s=1}^{\frac{T}{2}}$ such that 
    \begin{align*}
        Y_s = & \ell_{2s-1, c_{2s-1}}(a_{2s-1}) -  \ell_{2s-1, c_{2s-1}}(\pi_{c_{2s-1}}) \\
        &+ \ell_{2s, c_{2s}}(a_{2s}) -  \ell_{2s, c_{2s}}(\pi_{c_{2s}})  \\
        &- 2 \left( \widetilde{\ell}_{s,c_{s_{\ell}}}(a_{s_{\ell}}) - \widetilde{\ell}_{s,c_{s_{\ell}}}(\pi_{c_{s_{\ell}}}) \right).
        %& - \left( \ell_{2s-1, c_{2s-1}}(a_{2s-1}) -  \ell_{2s-1, c_{2s-1}}(\pi_{c_{2s-1}}) \right) \\
        %&-  \left( \ell_{2s, c_{2s}}(a_{2s}) -  \ell_{2s, c_{2s}}(\pi_{c_{2s}}) \right).
    \end{align*}
    % \left( \ell_{2s-1, c_{2s-1}}(a_{2s-1}) -  \ell_{2s-1, c_{2s-1}}(\pi_{c_{2s-1}}) \right) -  \left( \ell_{2s, c_{2s}}(a_{2s}) -  \ell_{2s, c_{2s}}(\pi_{c_{2s}}) \right) \}_{s=1}^{\frac{T}{2}}$.  
    Consider the filtration $\{\widetilde{H}_s\}_{s=1}^{\frac{T}{2}}$ such that for each $s$ the $\sigma$-field $\widetilde{H}_s$ is generated by the randomness within $c_t$ and $a_t$ for $t \le 2s$ and the randomness within sampling from pair $(2\tau-1,2\tau)$ for each $\tau \le s$. 
    %
    It is easy to see that the sequence$\{Y_s\}_{s=1}^{\frac{T}{2}}$  forms a martingale difference sequence adapted to the filtration $\{\widetilde{H}_s\}_{s=1}^{\frac{T}{2}}$. And it is also easy to see that $|Y_s| \le 2$.  Using Azuma-Hoeffding's inequality, for any constant $\delta \in (0,1)$ we have
    \[\sum_{s=1}^{\frac{T}{2}} Y_s  \le 2\sqrt{T \log(\frac{1}{\delta})} \]
    with probability at least $1 - \delta$.
    %
    That is exactly what we want to prove.
\end{proof}

Now we assume that we have already sampled the time step used in calculating loss estimates $t_{\ell}$ from pair $(t,t+1)$ for each $t = 1,3,\dots,T-1$. That is, we view the sequence of time steps used in calculating loss estimates $\{ t_{\ell}\}_{t=1,3,\dots,T-1}$ as an oblivious sequence.
%
We call the set of all time steps used in calculating loss estimates as $\Tl \triangleq \{ t_{\ell}\}_{t = 1,3,\dots,T-1}$, call the set of time steps in epoch $e$ used in calculating loss estimates as $\Tel \triangleq  \{ t_{\ell}\}_{t = (e-1)L+1,(e-1)L+3,\dots,eL-1}$. 
%
Note that once the time step used in calculating loss estimates $t_{\ell}$ is determined from pair $(t,t+1)$, the time step used in estimating frequency $t_f$ is accordingly determined as  the time step different from $t_{\ell}$ in pair $(t,t+1)$. Thus, we similarly call the set of all time steps used in estimating frequency $\Tf \triangleq \{ t_{f}\}_{t = 1,3,\dots,T-1}$, call the set of time steps in epoch $e$ used in estimating frequency as $\Tef \triangleq  \{ t_{f}\}_{t = (e-1)L+1,(e-1)L+3,\dots,eL-1}$
%
By \cref{lemma:used_loss_reduction}, we know that it suffices to bound the regret on the loss sequence used in calculating loss estimates 
\[\sum_{t \in \Tl} \ell_{t, c_t} (a_t) -  \ell_{t, c_t}(\pi_{c_{t}}). \]
%

We decompose it as follows.
\begin{align*}
&\sum_{t \in \Tl} \ell_{t, c_t} (a_t) -  \ell_{t, c_t}(\pi_{c_{t}}) \\
%
=& \sum_{t \in \Tl} \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -    \sum_c \Pr(c)  \left\langle p_{t,c} - \pi_c , \ell_{t,c} \right\rangle \right)  \\
&+  \sum_{t \in \Tl} \sum_c \Pr(c)  \left\langle p_{t,c} - \pi_c , \ell_{t,c} \right\rangle \\
%
% =& \sum_{t \in \Tl} \sum_c \Pr(c)  \left\langle p_{t,c} - \pi_c , \ell_{t,c} \right\rangle  \\
%  &+ \sum_{t \in \Tl} \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -    \sum_c \Pr(c)  \left\langle p_{t,c} - \pi_c , \ell_{t,c} \right\rangle \right) \\
%
=& \sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right) \\
&+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle\\
&+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle.
% % &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle\\
%  &+ \sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right).
% =& \sum_{t} \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle \\
%  &+ \sum_{t} \sum_{c} \Pr(c) \langle p_{t,c}, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle + \sum_{t} \sum_{c} \Pr(c) \langle \pi_c, \widehat{\ell}_{t,c} - l_{t,c} \rangle \\
%  &+ \sum_{t} \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right).
\end{align*}

In the previous decomposition, the term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$ is the bias term, and is the interesting one to bound. 
%
% [Zimmert 2023] decomposes the summand $ \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$  into three pieces and bound each piece separately.
% [Zimmert 2023] decomposes the summand $ \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$  into three pieces as follows:
% \begin{align*}
%      \left\langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \right\rangle =& \left\langle p_{t, c} - \pi_c, \ell_{t, c}-\widetilde{\ell}_{t, c} \right\rangle + \left\langle\widetilde{p}_{t, c}- \pi_c, \widetilde{\ell}_{t, c}-\widehat{\ell}_{t, c}\right\rangle\\
%      &+ \left\langle p_{t, c}-\widetilde{p}_{t, c}, \widetilde{\ell}_{t, c}-\widehat{\ell}_{t, c}\right\rangle.
% \end{align*}
We decompose the summand $\langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$ as follows:
\begin{align*}
     \left\langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \right\rangle =& \left\langle p_{t,c}, \ell_{t,c} - \widehat{\ell}_{t,c} \right\rangle + \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle \\
     %
     =& \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle  + \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle \\
      &+ \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle. \\
     % =& \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle \\
     %  &+ \left\langle \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle + \left\langle p_{t,c} - \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle  \\
     %  &+ \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle.
\end{align*}

% Our decomposition of the summand  $\langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$ is similar to the decomposition in [Zimmert 2023] but also different from it in a subtle but important manner. 
% %
% [Zimmert 2023] essentially decomposes term $\left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle$  into $\left\langle \pi_c, \widehat{\ell}_{t,c} - \widetilde{\ell}_{t,c} \right\rangle + \left\langle \pi_c, \widetilde{\ell}_{t,c} - \ell_{t,c} \right\rangle$ while we do not decompose term $\left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle$.
% %
% By keeping term $\left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle$ in its original form, we can add the term $\left\langle \pi_c, \widetilde{\ell}_{t,c} - \ell_{t,c} \right\rangle$  into our final bound. The term $\left\langle \pi_c, \widetilde{\ell}_{t,c} - \ell_{t,c} \right\rangle$  has negative expectation, which is crucial for our high probability bound.
% %We extract the inner product with $\pi_c$ out from $\left\langle p_{t, c} - \pi_c, \ell_{t, c}-\widetilde{\ell}_{t, c} \right\rangle + \left\langle\widetilde{p}_{t, c}- \pi_c, \widetilde{\ell}_{t, c}-\widehat{\ell}_{t, c}\right\rangle$ to form an independent term $\left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle$. By this extraction, 


% \begin{align*}
%      \left\langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \right\rangle =& \left\langle p_{t, c} - \pi_c, \ell_{t, c}-\widetilde{\ell}_{t, c} \right\rangle + \left\langle\widetilde{p}_{t, c}- \pi_c, \widetilde{\ell}_{t, c}-\widehat{\ell}_{t, c}\right\rangle\\
%      &+ \left\langle p_{t, c}-\widetilde{p}_{t, c}, \widetilde{\ell}_{t, c}-\widehat{\ell}_{t, c}\right\rangle.
% \end{align*}

Based on the decomposition of the summand, we further decompose the regret on the loss sequence used in calculating loss estimates into
\begin{align*}
    &\sum_{t \in \Tl} \ell_{t, c_t} (a_t) -  \ell_{t, c_t}(\pi_{c_{t}}) \\
    %  
    =& \sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right) \\
    &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle\\
    % &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle\\
    &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle \\
    &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle \\
    &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle. 
    % =& \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle\\
    % &+ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle\\
    % &+\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle \\
    % &+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle \\
    %   %&+ \sum_{t \in \Tl}\sum_{c} \Pr(c) \left\langle p_{t,c} - \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle  \\
    % &+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle \\
    % &+ \sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right).
\end{align*}
We bound these five summations one by one.

The first term \[\sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right) \]  is just a per-round concentration term, and is not hard to bound using Azuma-Hoeffding's inequality. 
%
The second term \[ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle \] and the third term \[ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle \] are also not hard to bound by applying techniques in the standard analysis of EXP3-IX. 
%
The remaining forth term \[ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle\] and fifth term \[\sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle\] are the two terms interesting to bound. We firstly focus on these two terms.


% In the above decomposition, the first term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle$ is not hard to bound using the standard analysis of EXP3-IX. The last term $\sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right)$ is just a per-round concentration term, and is also not hard to bound using Azuma-Hoeffding's inequality. We now focus on the middle term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$. 

% Given the previous decomposition, we can rewrite the term  $\sum_{t} \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \rangle$ as follows:
% \begin{align*}
%      \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c} - \pi_c, \ell_{t,c} - \widehat{\ell}_{t,c} \right\rangle =& \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle \\
%       &+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle \\
%       %&+ \sum_{t \in \Tl}\sum_{c} \Pr(c) \left\langle p_{t,c} - \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle  \\
%       &+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle.
% \end{align*}




% The first term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle $ is not hard to bound using standard EXP3-IX techniques. 
% %
% %The third term $ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c} - \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle $ is exactly the $\text{bias}_3$ term in [Zimmert 2023]. The argument in [Zimmert 2023] actually provides a high probability bound for it. 
% We now focus on the second term \[\sum_{t \in \Tl}\sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle\] and the third term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle$.

To bound these two terms, we will use the key observation mentioned in the begining of this section: different epochs in \Cref{alg:main}  are only weakly dependent from each other. To use  this observation rigorously, we introduce an important technological tool.
%
We define a filtration $\left\{ \His_e \right\}_e$, in which for each epoch $e$, the $\sigma$-algebra $\His_e$ is generated by all randomness in epoch $1,\dots,e-1$ and randomness in $\Tel$. That is, the $\sigma$-algebra $\His_e$ is generated precisely by the context $c_t$ and the random seed used in sampling $a_t \sim p_{t,c_t}$ for $t \le (e-1)L$ and $t \in \Tel$.
%
Note that for each epoch $e$, the  $\sigma$-algebra $\His_e$ excludes randomness in $\Tef$. This exclusion is crucial for characterizing the weak dependent structure between epochs. 

%into an atom random variable $\xi_e$. In another word, the atom random variable $\xi_e$ is made up precisely of the context $c_t$ and the random seed used in sampling $a_t \sim p_{t,c_t}$ for $t \in \mathcal{T}_{e-1}^f$ and $t \in \Tel$.
%
%It is easy to see that the set of random variables $\{\xi_e\}_e$ is mutually independent. 
%We will use this filtration to describe the weak dependent structure between epochs. 

\subsection{fifth}
We firstly bound the fifth term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle$. With a slight abuse of notations, we define a filtration $\{\His_t\}_t$ such that the  $\sigma$-algebra $\His_t$ for each time step $t$ is generated by all randomness before time $t$. 
%
We decompose the fifth term into two terms:
\begin{align*}
&\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle\\
%
=& \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) - \ell_{t,c}(\pi_c) \right)\\
%
=&  \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right]- \ell_{t,c}(\pi_c) \right) \\
&+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right).
% %
% =& \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right)\\
% &+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right]- \ell_{t,c}(\pi_c) \right).
\end{align*}
We bound the two terms separately.

%The first term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right]- \ell_{t,c}(\pi_c) \right)$.
%
%It equals \[\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \frac{f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} \right) \ell_{t,c}(\pi_c) .\]
%
For each epoch $e$, we define a random variable 
\[\BiasFifth_e \triangleq \sum_{t \in \Tel} \sum_{c} \Pr(c)  \left( \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right]- \ell_{t,c}(\pi_c) \right).\] 
%
We rewrite the first term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right]- \ell_{t,c}(\pi_c) \right)$ as $\sum_{e=1}^{T/L} \BiasFifth_e$.
%
Recall our key observation: different epochs are only weakly dependent from each other. We bound the summation over epochs $\sum_{e=1}^{T/L} \BiasFifth_e$ by leveraging the weak dependent structure between $\left\{\BiasFifth_e\right\}_e$. 
%
% Further more, following terminology in [Zimmert 2023], we consider a sequence of indicator function $\{ F_e \}_e$ such that \[F_e \triangleq \indi \left( \forall k, \left|\widehat{f}_{e}(k)-f_{e}(k)\right| \leq 2 \max \left\{\sqrt{\frac{f_{e}(k) \iota}{L}}, \frac{\iota}{L}\right\} \right).\]
% %
% Thissequence of random variables and another sequence of random variables $\{\BiasFifth_e\}_e$ have the following properties:


The sequence of random variables $\{\BiasFifth_e\}_e$ has 
the following properties:
\begin{enumerate}
    \item For each epoch $e$, the random variable $ \BiasFifth_e$ is measurable under $\sigma$-algebra $\His_e$.
    % and $F_e$ are functions of first $e$ atom random variables $\xi_1,\dots,\xi_e$.
    %
    %\item For each epoch $e$, we have 
    %    \[\E\left[ F_e \big| \His_{e-1} \right] \ge 1-2 K \exp (-\iota). \]
    %
    \item For each epoch $e$, we have
        \begin{align*}
            &\E\left[ \BiasFifth_e \cdot F_e \big| \His_{e-1} \right]\\
            =& \sum_c \Pr(c) \sum_{t \in \Tel} \ell_{t,c}(\pi_c) \E\left[ \left( \frac{f_e(\pi_c)}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} - 1 \right) F_e \big| \His_{e-1} \right].
            % =& \sum_c \Pr(c) \sum_{t \in \Tel} \ell_{t,c}(\pi_c) \E\left[ \left( \frac{f_e(\pi_c)}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} -  \frac{f_e(\pi_c)}{f_e(\pi_c) + \gamma} +\frac{f_e(\pi_c)}{f_e(\pi_c) + \gamma} - 1 \right) F_e \big| \His_{e-1} \right]
        \end{align*}
    We further have 
    \begin{align*}
        &\E\left[ \left( \frac{f_e(\pi_c)}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} - 1 \right) F_e \big| \His_{e-1} \right]\\
        =& \E\left[ \left( \frac{f_e(\pi_c)}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} -  \frac{f_e(\pi_c)}{f_e(\pi_c) + \gamma} +\frac{f_e(\pi_c)}{f_e(\pi_c) + \gamma} - 1 \right) F_e \big| \His_{e-1} \right] \\
        =& \E\left[ \frac{f_e(\pi_c)}{f_e(\pi_c)+\gamma}  \frac{\left(f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{1}{2} \gamma \right)}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} F_e \big| \His_{e-1}  \right] - \frac{\gamma}{f_e(\pi_c) + \gamma} \E\left[F_e \big| \His_{e-1}  \right] \\
        \le& - \frac{\gamma}{f_e(\pi_c) + \gamma} \E\left[F_e \big| \His_{e-1}  \right]\\
        \le&  - \frac{\gamma}{f_e(\pi_c) + \gamma} \left(  1-2 K \exp (-\iota) \right).
    \end{align*}
    Here in the first inequality we use Lemma10 in [Zimmert 2023]. Thus we have
    \begin{align*}
        &\E\left[ \BiasFifth_e \cdot F_e \big| \His_{e-1} \right]\\
        %
        \le& - \sum_c \Pr(c) \sum_{t \in \Tel} \ell_{t,c}(\pi_c)\frac{\gamma}{f_e(\pi_c) + \gamma} \left(  1-2 K \exp (-\iota) \right).
    \end{align*}
    %
  \item For each epoch $e$, we have
    \begin{align*}
        \BiasFifth_e F_e &\le  \sum_{c} \Pr(c) \sum_{t \in \Tel} \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] F_e \\
        &= \sum_{c} \Pr(c) \sum_{t \in \Tel} \ell_{t,c}(\pi_c) \frac{f_e(\pi_c)}{\widehat{f}_e(\pi_c) + \frac{3}{2}\gamma} F_e \\
        &\le \sum_{c} \Pr(c) \sum_{t \in \Tel} \ell_{t,c}(\pi_c) \frac{2 f_e(\pi_c)}{f_e(\pi_c) + \gamma} \\
        &\le 2 L \le \frac{32\iota}{\gamma}.
    \end{align*}
    \item For each epoch $e$, we have
    %\big| \His_{e-1}
    \begin{align*}
        &\E\left[ (\BiasFifth_e F_e)^2 \big| \His_{e-1}\right]\\ 
        =& \E\left[\left(\sum_{c} \Pr(c) \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \frac{f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma }{ \widehat{f}_e(\pi_c) + \frac{3}{2} \gamma} F_e \right)^2 \big| \His_{e-1} \right]\\
        &\le \sum_c \Pr(c) \E\left[\left(\sum_{t \in \Tel} \ell_{t,c}(\pi_c) \frac{f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma }{ \widehat{f}_e(\pi_c) + \frac{3}{2} \gamma} F_e \right)^2 \big| \His_{e-1} \right]\\
        &=  \sum_c \Pr(c) (\sum_{t \in \Tel} \ell_{t,c})^2 \E\left[ \left( \frac{f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma }{ \widehat{f}_e(\pi_c) + \frac{3}{2} \gamma} F_e \right)^2\big| \His_{e-1}\right] \\
        %&= (\sum_{t \in T_e} l_{t,c}(a))^2 \Var[\frac{p_e(a) - \widehat{p}_e(a) -\frac{3}{2}\gamma}{ \widehat{p}_e(a) + \frac{3}{2} \gamma}|H_{e-1}] \\
        &\le L  \sum_c \Pr(c) \sum_{t \in \Tel} \ell_{t,c} \E\left[ \left( \frac{f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma }{ \widehat{f}_e(\pi_c) + \frac{3}{2} \gamma} F_e \right)^2\big| \His_{e-1}\right] \\
        %·  &\le L \sum_{t \in T_e}  l_{t,c}(a)  \E[(\frac{p_e(a) - \widehat{p}_e(a) -\frac{3}{2}\gamma}{ \widehat{p}_e(a) + \frac{3}{2} \gamma})^2 | H_{e-1}] \\
        %
        &\le 4 L \sum_c \Pr(c) \sum_{t \in \Tel} \ell_{t,c} \E\left[\left( \frac{f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma }{ f_e(\pi_c) + \gamma} F_e \right)^2\big| \His_{e-1} \right]\\
        &\le \sum_c \Pr(c)  \frac{4 L}{(f_e(\pi_c) + \gamma)^2} \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \E\left[ \left(f_e(\pi_c) - \widehat{f}_e(\pi_c) - \frac{3}{2}\gamma \right)^2 \big| \His_{e-1} \right] \\
        &= \sum_c \Pr(c) \frac{4 L}{(f_e(\pi_c) + \gamma)^2} \sum_{t \in \Tel}   \ell_{t,c}(\pi_c) \left(\E\left[ \left(f_e(\pi_c) - \widehat{f}_e(\pi_c)\right)^2 \big| \His_{e-1} \right] + \frac{9}{4}\gamma^2 \right) \\
        &\le \sum_c \Pr(c) \frac{4 L}{(f_e(\pi_c) + \gamma)^2} \sum_{t \in \Tel}  \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \left(\frac{f_e(\pi_c)}{L}+ \frac{9}{4}\gamma^2 \right) \\
        &\le 4 \sum_c \Pr(c) \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \left( \frac{1}{f_e(\pi_c) + \gamma} + \frac{9L \gamma }{4(f_e(\pi_c) + \frac{3}{2}\gamma)} \right) \\
        &\le 4 \sum_c \Pr(c) \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) + \gamma}.
    \end{align*}
\end{enumerate}

Given these properties, we use Freedman's inequality to get that for any $0 < \lambda <\frac{ \gamma}{32\iota}$, with probability at least $1- \delta$, we have
\[\sum_e \BiasFifth_e F_e - \E[\BiasFifth_e F_e \big| \His_{e-1}]  \le 4 \lambda \sum_c \Pr(c) \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) + \frac{3}{2} \gamma} + \frac{\log(1/\delta)}{\lambda}. \] 
We further have that event $\{ \sum_e \BiasFifth_e F_e = \sum_e \BiasFifth_e \}$ holds if event $G$ holds.
%
Combining  these two facts, we get that the inequality
\[\sum_e \BiasFifth_e  - \E[\BiasFifth_e F_e \big| \His_{e-1}]  \le 4 \lambda \sum_c \Pr(c) \sum_{t \in \Tel}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) + \gamma} + \frac{\log(1/\delta)}{\lambda} \]
holds with probability at least $\Pr(G) - \delta$.

We now bound the second term \[\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right).\]
%
The second term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right)$ having following properties:
\begin{enumerate}
    \item The sequence of random variables $\left\{ \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right)\right\}_{t \in \Tl}$ forms a martingale difference sequence with respect to filtration $\{ \His_t \}_t$.
    \item Each random variable $\sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right) $ satisfies $ \left| \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right) \right| \le \frac{1}{\gamma}$.
    \item Each random variable $\sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right)$ satisfies
        \begin{align*}
        \Var \left[ \sum_{c} \Pr(c)\widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] &\le \sum_{c} \Pr(c) \Var\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \\
        &= \sum_{c} \Pr(c)  \frac{f_e(\pi_c) - f^2_e(\pi_c)}{\left(\widehat{f}_e(\pi_c)+ \frac{3}{2} \gamma \right)^2} l_{t, c}(\pi_c)^2  \\
        &\le  \sum_{c} \Pr(c)  \frac{f_e(\pi_c)}{\left(\widehat{f}_e(\pi_c)+ \frac{3}{2} \gamma \right)^2} l_{t, c}(\pi_c).
        \end{align*}
\end{enumerate}

Applying Freedman's inequality on the sequence of random variables $\left\{ \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right)\right\}_{t \in \Tl}$ , we get that for each $\delta \in (0,1)$ and each $0 < \lambda < \gamma$, with probability at least $1 - \delta$, we have
\begin{align*}
    &\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right) \\
    \le& \lambda \sum_{t \in \Tl}  \sum_{c} \Pr(c)  \frac{f_e(\pi_c)}{\left(\widehat{f}_e(\pi_c)+ \frac{3}{2} \gamma \right)^2} l_{t, c}(\pi_c) + \frac{1}{\lambda} \log(\frac{1}{\delta}).
\end{align*}
By assuming event $G$ holds, we further get  that with probability at least $\Pr(G) - \delta$ the following inequality holds
\begin{align*}
    &\sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right) \\
    \le& 4 \lambda \sum_{t \in \Tl}  \sum_{c} \Pr(c)  \frac{f_e(\pi_c)}{\left(f_e(\pi_c)+ \gamma \right)^2} l_{t, c}(\pi_c) + \frac{1}{\lambda} \log(\frac{1}{\delta}).
\end{align*}

Combining all previous inequalities, we get that for any $0 < \lambda_1 <\frac{ \gamma}{32\iota}$ and $0 < \lambda_2 < \gamma$ , the following inequality holds with probability at least $\Pr(G) - 2\delta $:
\begin{align*}
&\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle\\
%
=& \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right]- \ell_{t,c}(\pi_c) \right)  \\
&+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right) \\
%
=& \sum_e \BiasFifth_e  - \E[\BiasFifth_e F_e \big| \His_{e-1}] \\
&+ \sum_e \E\left[\BiasFifth_e F_e \big| \His_{e-1}\right] \\
&+  \sum_{t \in \Tl} \sum_{c} \Pr(c) \left( \widehat{\ell}_{t,c}(\pi_c) -  \E\left[ \widehat{\ell}_{t,c}(\pi_c) \big| \His_{t-1} \right] \right)\\
%
\le& 4 \lambda_1 \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) +  \gamma} + \frac{\log(1/\delta)}{\lambda_1} \\
&- \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{\gamma}{f_e(\pi_c) + \gamma} \left(  1-2 K \exp (-\iota) \right) \\
&+ 4 \lambda_2 \sum_{t \in \Tl}  \sum_{c} \Pr(c)  \frac{f_e(\pi_c)}{\left(f_e(\pi_c) +  \gamma \right)^2} l_{t, c}(\pi_c) + \frac{1}{\lambda_2} \log(\frac{1}{\delta}).
% %
% \le&  2 \lambda_1 \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{1}{f_{e}(\pi_c) + \gamma} + \frac{1}{\lambda_1 } \log(1/\delta)\\
% &+ 4\lambda_2   \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) + \frac{3}{2} \gamma} + \frac{\log(1/\delta)}{\lambda_2} \\
% &- \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{\gamma}{f_e(\pi_c) + \gamma} \left(  1-2 K \exp (-\iota) \right). \\  
\end{align*}

Note that in the previous analysis, we combine two good events each happening with probability at least $\Pr(G) - \delta$. The combined good event happens with probability $\Pr(G) - 2\delta$ rather than the vanilla union bound $1 - 2(1-\Pr(G) + \delta)$. This is because in both events the $\Pr(G)$ term comes from assuming event $G$ happens. Thus in the combined event we can just assume event $G$ happens and only count the corresponding bad event $G^c$ once. We will use this small trick repeatedly in following analysis.

We pick $\lambda_1 = \frac{\gamma}{8 \cdot 36 \iota}$ and $\lambda_2 = \frac{\gamma}{8} $  to get that the following inequality holds with probability at least $\Pr(G) - 2\delta)$:
\begin{align*}
&\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle \pi_c, \widehat{\ell}_{t,c} - \ell_{t,c} \right\rangle \\
%
\le& 4 \lambda_1 \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) +  \gamma} + \frac{\log(1/\delta)}{\lambda_1} \\
&- \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{\gamma}{f_e(\pi_c) + \gamma} \left(  1-2 K \exp (-\iota) \right) \\
&+ 4 \lambda_2 \sum_{t \in \Tl}  \sum_{c} \Pr(c)  \frac{f_e(\pi_c)}{\left(f_e(\pi_c) +  \gamma \right)^2} l_{t, c}(\pi_c) + \frac{1}{\lambda_2} \log(\frac{1}{\delta}) \\
% %
% \le&  2 \lambda_1 \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{1}{f_{e}(\pi_c) + \gamma} + \frac{1}{\lambda_1 } \log(1/\delta)\\
% &+ 4\lambda_2   \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{36\iota}{f_e(\pi_c) + \frac{3}{2} \gamma} + \frac{\log(1/\delta)}{\lambda_2} \\
% &- \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c) \frac{\gamma}{f_e(\pi_c) + \gamma} \left(  1-2 K \exp (-\iota) \right) \\
% %
=& (\frac{8 \cdot 36 \iota}{\gamma} + \frac{8}{\gamma}) \log(1/\delta) +  \sum_c \Pr(c) \sum_{t \in \Tl}  \ell_{t,c}(\pi_c)  \frac{\gamma}{f_e(\pi_c) + \gamma} 2K \exp(-\iota)\\
%
\le& (\frac{8 \cdot 36 \iota}{\gamma} + \frac{8}{\gamma}) \log(1/\delta) + KT \exp(-\iota).
\end{align*}

\subsection{forth}
We then bound the forth term $\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle$. Similar to the previous analysis, we decompose it as follows:
\begin{align*}
    &\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle\\
    %
    =&\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle\\
    &+\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle .
\end{align*}
We bound these two terms separately.

Similar to the previous anlaysis, we decompose the first term \[\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle\] as \[\sum_{e} \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle p_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle.\]
%
For each epoch $e$ we define a random variable 
\[\BiasSecond_e \triangleq \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle p_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle.\]
%
We need to bound $\sum_e \BiasSecond_e$.

We decompose $\sum_e \BiasSecond_e$ as $\sum_e \BiasSecond F_eL_e + \sum_e \BiasSecond_e (1- F_eL_e)$. 
%
As usual we have that $\sum_e \BiasSecond_e (1- F_eL_e) = 0$ whenever event $G$ holds. 
%
Thus we can focus on bounding $\sum_e \BiasSecond_e F_eL_e$. 
%
Firstly we bound \[\sum_e \E\left[ \BiasSecond_e F_e L_e \big| \His_{e-1} \right].\]

We have 
\begin{align*}
    &\sum_e \E\left[ \BiasSecond_e F_e L_e \big| \His_{e-1} \right] \\
    %
    =&  \sum_{e} \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e L_e \big| \His_{e-1} \right]\\
    &+ \sum_{e} \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle p_{t,c} - \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e L_e \big| \His_{e-1} \right].
\end{align*}
%

[Zimmert 2023] showed that the latter term \[\sum_{e} \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle p_{t,c} - \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e L_e \big| \His_{e-1} \right]\] is bounded by  $\frac{98 K T \iota}{L}+\frac{\gamma^2 L K T}{\iota}.$ 
%
Furthermore, condition on $\His_{e-1}$, the indicator function $F_e$ is effected only by randomness within time steps $t \in \Tef$, thus the indicator function $F_e$ is conditional independent with the probability vector $\widetilde{p}_{t,c}$. 
%
We have 
\begin{align*}
    &\sum_e \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e \big| \His_{e-1} \right]\\
    %
    =& \sum_e \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle \E\left[ \widetilde{p}_{t,c} \big| \His_{e-1} \right], \E\left[ (\widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c}) F_e \big| \His_{e-1} \right] \right\rangle \\
    \le& \sum_e \sum_{t \in \Tel} \sum_{c} \Pr(c) \sum_a \frac{\widetilde{p}_{t, c}(a) \gamma}{f_{e}(a)}.
\end{align*}

Whenever event $G$ holds, the ratio $\frac{\widetilde{p}_{t, c}(a)}{f_{e}(a)} \le 4.$ Thus we have \[\sum_e \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e \big| \His_{e-1} \right] \le 4 \gamma K  T\] whenever event $G$ holds.


% [Zimmert 2023] showed that
% \[\sum_e \E\left[ \BiasSecond_e F_e \big| \His_{e-1} \right] \le 4 K \gamma T + \frac{98 K T \iota}{L}+\frac{\gamma^2 L K T}{\iota} . \]
% %
We further have $\left| \left\langle \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \right| \le \frac{1}{\gamma}$.
%
Thus we have
\begin{align*}
    & \sum_e \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e (L_e-1) \big| \His_{e-1} \right]  \\
    %
    \le& \sum_e \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \frac{1}{\gamma} F_e (L_e-1) \big| \His_{e-1} \right]  \\
    %
    \le& \frac{1}{\gamma} \sum_e \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c)  \left| L_e - 1 \right| \big| \His_{e-1} \right]  \\
    %
    % \le& \left| \sum_e \left|\E\left[ (L_e-1)|\His_{e-1} \right]\right| \frac{1}{\gamma} \right| \\
    %
    \le& \frac{K \exp(-\iota) T}{\gamma} .
\end{align*}


% \begin{align*}
% &\left|\sum_e \E\left[ \BiasSecond_e F_e (1-L_e) \big| \His_{e-1} \right]\right| \\
% %
% \le& \left| \sum_e \left|\E\left[ (1-L_e)|\His_{e-1} \right]\right| \frac{1}{\gamma} \right| \\
% %
% \le& K \exp(-\iota) \frac{T}{\gamma}.
% \end{align*}
% %\[\left|\sum_e \E\left[ \BiasSecond_e F_e (1-L_e) \big| \His_{e-1} \right]\right| \le \Pr(G) \frac{T}{\gamma}. \]
% %
Thus we have 
\begin{align*}
   &\sum_e \E\left[ \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_eL_e \big| \His_{e-1} \right]\\
   %
   \le& 4 \gamma K  T +  \frac{K \exp(-\iota) T}{\gamma} 
\end{align*}
whenever event $G$ holds.

Thus we have
\[\sum_e \E\left[ \BiasSecond_e F_e L_e \big| \His_{e-1} \right] \le4 K \gamma T +  \frac{K \exp(-\iota) T}{\gamma} + \frac{98 K T \iota}{L}+\frac{\gamma^2 L K T}{\iota} \]
whenever event $G$ holds.

We then only need to bound the concentration term \[\sum_e \BiasSecond_e F_e L_e- \E\left[ \BiasSecond_e F_e L_e \big| \His_{e-1} \right].\]

For each random variable $\BiasSecond_e F_e L_e $, we have

\begin{align*}
    &\BiasSecond_e F_e L_e\\
    %
    =& \sum_{t \in \Tel} \sum_{c} \Pr(c) \left\langle p_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e L_e\\
    %
     =& \sum_{t \in \Tel} \sum_{c} \Pr(c) \sum_a p_{t,c}(a) f_e(a) \ell_{t,c}(a) \left( \frac{1}{f_e(a) + \gamma} - \frac{1}{\widehat{f}_e(a) + \frac{3}{2} \gamma} \right) F_e L_e \\
     %
    =& \sum_{t \in \Tel} \sum_{c} \Pr(c) \sum_a \widetilde{p}_{t,c}(a) f_e(a) \ell_{t,c}(a) \frac{\widehat{f}_e(a) - f_e(a) + \frac{1}{2}\gamma}{(f_e(a) + \gamma)(\widehat{f}_e(a) + \frac{3}{2} \gamma)} F_e L_e.\\
    %
    % &\sim \\
    % % &= \sum_{t \in T_e} \sum_{c} \Pr(c) \sum_{a}  \widetilde{p}_{t,c}(a) \E[ \widetilde{l}_{t,c}(a) - \widehat{\ell}_{t,c}(a) | H_{t-1}] \\
    % %
    % % &= \sum_{t \in T_e} \sum_{c} \Pr(c) \sum_a \widetilde{p}_{t,c}(a) p_t(a) l_{t,c}(a) [ \frac{1}{p_t(a) + \gamma} - \frac{1}{\widehat{p}_t(a) + \frac{3}{2} \gamma}] \\
    % &=  \sum_{t \in T_e} \sum_{c} \Pr(c) \sum_a   \widetilde{p}_{t,c}(a) p_t(a) l_{t,c}(a) \frac{\widehat{p}_t(a) - p_t(a) + \frac{3}{2} \gamma }{(p_t(a) + \gamma)(\widehat{p}_t(a) + \frac{1}{2} \gamma)}  \\
    % &\sim \sum_{t \in T_e} \sum_{c} \Pr(c)  \widetilde{p}_{t,c}(a_t) \frac{\sqrt{\frac{p_t(a_t)}{\sqrt{KT}}} + \frac{3}{2} \gamma }{(p_t(a_t) + \gamma)(\widehat{p}_t(a_t) + \frac{3}{2} \gamma)} \\
    % &\sim \sum_{t \in T_e}  \frac{\sqrt{\frac{p_t(a_t)}{\sqrt{KT}}}}{(p_t(a_t) + \gamma)}
\end{align*}

Thus we have
\begin{align*}
    &\left| \BiasSecond_e F_eL_e \right|\\
    %
    \le& \left| \sum_{t \in \Tel} \sum_{c} \Pr(c) \sum_a \widetilde{p}_{t,c}(a) f_e(a) \ell_{t,c}(a)  \frac{\widehat{f}_e(a) - f_e(a) + \frac{1}{2}\gamma}{(f_e(a) + \gamma)(\widehat{f}_e(a) + \frac{3}{2} \gamma)} \right| F_eL_e \\
    %
    \le& \sum_{t \in \Tel} \sum_a \widetilde{p}_{t}(a) \left| \frac{\widehat{f}_e(a) - f_e(a) + \frac{1}{2}\gamma}{\widehat{f}_e(a) + \frac{3}{2} \gamma}  \right| F_eL_e \\
    %
    %\le& 2 \sum_{t \in \Tel} \sum_a \widetilde{p}_{t}(a) \frac{2 \max \left\{\sqrt{\frac{f_{e}(a) \iota}{L}}, \frac{\iota}{L} \right\}}{f_e(a) + \gamma}\\
    %
    \le& 8  \sum_{t \in \Tel} \sum_a \max \left\{\sqrt{\frac{f_{e}(a) \iota}{L}}, \frac{\iota}{L} \right\}\\
    %
    \le& 8 L (\sqrt{\frac{K\iota}{L}} + \frac{K\iota}{L})\\
    %
    =&   8(\sqrt{KL\iota} + K\iota).
\end{align*}

Applying Azuma-Hoeffding's inequality on \[\sum_e  \BiasSecond_e F_eL_e -  \E\left[\BiasSecond_e F_eL_e \big| \His_{e-1} \right],\] 
%
we get that for any $\delta > 0$,  with probability at least $1 - \delta$ we have
\begin{align*}
    &\sum_e  \BiasSecond_e F_eL_e -  \E\left[\BiasSecond_e F_eL_e \big| \His_{e-1} \right]\\
    %
    \le&  8(\sqrt{KL\iota} + K\iota)\sqrt{2\frac{T}{L}\log(\frac{\delta}{2})} \\
    %
    =& 8\left(\sqrt{2KT\iota \log(\frac{\delta}{2})} + \sqrt{2\frac{TK^2}{L}\iota \log(\frac{\delta}{2})}\right).
\end{align*}

Thus we have 
\begin{align*}
    &\sum_e  \BiasSecond_e F_eL_e \\
    %
    \le& 4 K \gamma T +  \frac{K \exp(-\iota) T}{\gamma} + \frac{98 K T \iota}{L}+\frac{\gamma^2 L K T}{\iota} \\
    &+ 8\left(\sqrt{2KT\iota \log(\frac{\delta}{2})} + \sqrt{2\frac{TK^2}{L}\iota \log(\frac{\delta}{2})}\right).
\end{align*}
with probability at least $\Pr(G) - \delta$.

We then bound the second term \[\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle.\] 
%
For each time step $t \in \Tel$, we define an indicator function \[\widetilde{L}_t \triangleq \indi\left(\forall a, \widetilde{p}_{t}(a) \le 4 f_e(a) \right).\] Note that event $G$ implies $\forall t \in \Tel, \widetilde{L}_t = 1.$

Similar to previous analysis, we decompose the first term as
\begin{align*}
    &\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \\
    %
    =&\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e\widetilde{L}_t \\
    &+ \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle (1-F_e \widetilde{L}_t).
\end{align*}

Since the auxiliary probability vector $\widetilde{p}_{t,c}$ is determined at time $t-1$, the indicator function $\widetilde{L}_t$ is also determined at time $t-1$. 
%
Furthermore, the indicator function $F_e$ is determined at epoch $e-1$.
%
Thus the product of indicator functions $F_e \widetilde{L}_t$ is measurable under filtration $\His_{t-1}$. We have
\begin{align*}
    &\E\left[\sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e \widetilde{L}_t\big| \His_{t-1} \right]\\
    %
    =& F_e\widetilde{L}_t \E\left[  \sum_{c} \Pr(c) \left\langle p_{t,c}, (\widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c})  - \E\left[ (\widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c}) \big| \His_{t-1} \right] \right\rangle \big| \His_{t-1} \right] \\
    %
    =& 0.
\end{align*}
Thus the sequence of random variables \[\left\{ \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e \widetilde{L}_t \right\}_{t \in \Tl}\] forms an MDS under filtation $\{\His_t\}_t$.

We further have that the term 
\[\sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e\widetilde{L}_t \] satisfies
% \begin{enumerate}
%     \item The sequence of random variables \[\left\{\sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \right\}_{t \in \Tl}\] forms a martingale difference sequence with respect to filtration $\{ \His_t \}_t$.
%     %
%     \item  Each random variable satisfies 
    \begin{align*}
        &\left| \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \right| F_e\widetilde{L}_t \\
        %
        \le& \left| \sum_{c} \Pr(c) \sum_{a} p_{t,c}(a) \ell_{t,c}(a) \left(  \frac{\indi(a_t = a)}{f_e(a) + \gamma} -  \frac{f_e(a)}{f_e(a) + \gamma}\right) \right| F_e\widetilde{L}_t \\
        &+ \left|\sum_{c} \Pr(c) \sum_{a} p_{t,c}(a) \ell_{t,c}(a) \left(  \frac{\indi(a_t = a)}{\widehat{f}_e(a) + \frac{3}{2}\gamma} -  \frac{f_e(a)}{\widehat{f}_e(a) + \frac{3}{2}\gamma}\right) \right| F_e\widetilde{L}_t \\
        %
        \le& \sum_{c} \Pr(c) p_{t,c}(a_t) \frac{\ell_{t,c}(a_t) }{f_e(a_t) + \gamma} F_e\widetilde{L}_t \\
        &+ \sum_{c} \Pr(c) \sum_{a} p_{t,c}(a) \ell_{t,c}(a) \frac{f_e(a)}{f_e(a) + \gamma} F_e\widetilde{L}_t \\
        &+ \sum_{c} \Pr(c) p_{t,c}(a_t) \frac{\ell_{t,c}(a_t) }{\widehat{f}_e(a_t) + \frac{3}{2} \gamma} F_e \widetilde{L}_t\\
        &+ \sum_{c} \Pr(c) \sum_{a} p_{t,c}(a) \ell_{t,c}(a) \frac{f_e(a)}{\widehat{f}_e(a) + \frac{3}{2}\gamma} F_e\widetilde{L}_t \\
        %
        \le& \left( \frac{p_t(a_t)}{f_e(a_t) + \gamma} + 1 +  \frac{p_t(a_t)}{\widehat{f}_e(a_t) + \frac{3}{2}\gamma} + \sum_{a} p_t(a) \frac{f_e(a)}{\widehat{f}_e(a) + \frac{3}{2}\gamma} \right) F_e \widetilde{L}_t\\
        %
        \le& 4+1+8+2 = 15.
    \end{align*}
    % %
    % \item Each random variable satisfies 
    % \[\sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \le \frac{2}{\gamma}\].
    % %
    % \item Each random variable \[\sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle\] satisfies
    %     \begin{align*}
    %     &\Var \left[ \sum_{c} \Pr(c) \left\langle \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c}  \right\rangle \big| \His_{t-1} \right]\\
    %     %
    %     \le& \sum_{c} \Pr(c) \Var\left[ \left\langle \widetilde{p}_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c}  \right\rangle \big| \His_{t-1} \right] \\
    %     %
    %     \le & \sum_{c} \Pr(c) \sum_{a} \widetilde{p}_{t,c}(a) \Var\left[ \widetilde{l}_{t,c}(a) - \widehat{l}_{t,c}(a) \big| \His_{t-1} \right]\\
    %     %
    %     =& \sum_{c} \Pr(c) \sum_{a} \widetilde{p}_{t,c}(a) \ell^2_{t,c}(a) \left( f_e(a) - f^2_e(a) \right) \left(\frac{1}{f_e(a) + \gamma} + \frac{1}{\widehat{f}_e(a) + \frac{3}{2} \gamma} \right)^2\\
    %     %
    %     \le& \sum_{a} \widetilde{f}_e(a) f_e(a) \left( (\frac{1}{(f_e(a) + \gamma)^2} + \frac{1}{(\widehat{f}_e(a) + \frac{3}{2} \gamma)^2} + \frac{1}{(\widehat{f}_e(a) + \frac{3}{2} \gamma)(f_e(a) + \gamma)}  \right). \\
    %     \end{align*}
%\end{enumerate}

%The product of indicator functions $F_e$ has two properties. Firstly, it is measurable under filtration $\His_{t-1}$. Secondly, event $G$ implies event $\{F_e = 1\}$. Thus we have

Applying Azuma-Hoeffding's inequality on the sequnece of random variables
%
\[\left\{ \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e\widetilde{L}_t \right\}_{t \in \Tl},\]
%
we get that for any $\delta > 0$,
%
the inequality
\[   \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle F_e \widetilde{L}_t \le 15 \sqrt{T\log(\frac{1}{\delta})}\] 
%
holds with probability at least $1- \delta$.

On the other hand, note that event $G$ implies event $\{F_e \widetilde{L}_t = 1 \}$, we get that 
\[\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle (1-F_e\widetilde{L}_t) = 0 \]
whenever event $G$ holds. Thus we get that for any $\delta > 0$, inequality
\[  \sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \le 15 \sqrt{T\log(\frac{1}{\delta})}\] 
holds with probability at least $\Pr(G) - 2\delta$.

Combining previous results, we get that the following inequality holds with probability at least $\Pr(G) - 2\delta$:
\begin{align*}
    &\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \right\rangle\\
    %
    =&\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle\\
    &+\sum_{t \in \Tl} \sum_{c} \Pr(c) \left\langle p_{t,c}, \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} - \E\left[ \widetilde{\ell}_{t,c} - \widehat{\ell}_{t,c} \big| \His_{t-1} \right] \right\rangle \\
    %
    \le& 4 K \gamma T +  \frac{K \exp(-\iota) T}{\gamma} + \frac{98 K T \iota}{L}+\frac{\gamma^2 L K T}{\iota} \\
    &+ 8\left(\sqrt{2KT\iota \log(\frac{\delta}{2})} + \sqrt{2\frac{TK^2}{L}\iota \log(\frac{\delta}{2})}\right)\\
    &+  15 \sqrt{T\log(\frac{1}{\delta})}.
\end{align*}

\subsection{first, second and third}

The remaining terms are the first, second and third term. These terms are easy to bound by applying techniques in standard EXP3-IX analysis. We write down these analysis in the sake of completeness. 

\subsubsection{first}
Here we bound the first term  \[\sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right). \] 

Whenever event $G$ holds, we have $q_t = p_t$. Thus we assume event $G$ holds and replace the original term with \[\sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle q_{t,c} - \pi_c , \ell_{t,c} \rangle \right). \] 

The new term have the following properties:
\begin{itemize}
    \item The sequence of summands \[\left\{ \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle q_{t,c} - \pi_c , \ell_{t,c} \rangle \right\}_{t \in \Tl}\] adapts to the filtration $\left\{\His_t\right\}_{t \in \Tl}$.
    \item The sequence of summands satisfies \[\E\left[\ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle q_{t,c} - \pi_c , \ell_{t,c} \rangle \big| \His_{t-1} \right] = 0.\]
    \item Each summand $ \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle q_{t,c} - \pi_c , \ell_{t,c} \rangle\in [-2,2]$. 
\end{itemize}

By applying Azuma-Hoeffding inequality, we get that for any $\delta \in (0,1)$, the following inequality holds with probability at least $1 - \delta$:
\begin{align*}
    &\sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle q_{t,c} - \pi_c , \ell_{t,c} \rangle \right)\\
    %
    \le& 2 \sqrt{T \log(\frac{1}{\delta})}
\end{align*}
Thus the following inequality holds with probabiity at least $\Pr(G) - \delta$:
\[\sum_{t \in \Tl}  \left( \ell_{t, c_{t}}(a_{t}) -  \ell_{t, c_{t}}(\pi_{c_{t}})  -   \sum_c \Pr(c)  \langle p_{t,c} - \pi_c , \ell_{t,c} \rangle \right) \le 2 \sqrt{T \log(\frac{1}{\delta})}.\]

\subsubsection{second}
Here we bound the second term  \[ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle. \]

The second term satisfies
\begin{align*}
    &\sum_{t \in \Tl}  \sum_{c} \Pr(c) \langle p_{t,c} - \pi_c, \widehat{\ell}_{t,c} \rangle\\
    %
    \le&\sum_{c} \Pr(c) \left( \frac{1}{\eta} \log K  + \frac{\eta}{2} \sum_{t \in \Tl} \left\langle p_{t,c}, \widehat{\ell}^2_{t,c} \right\rangle \right).
    %
\end{align*}

When event $G$ holds, we have $\widehat{\ell}_{t,c} \le 2 \widetilde{\ell}_{t,c}$. Thus assuming event $G$ holds, we can focus on upper bounding \[\sum_{c} \Pr(c) \left( \frac{1}{\eta} \log K  + 2 \eta \sum_{t \in \Tl} \left\langle p_{t,c}, \widetilde{\ell}^2_{t,c} \right\rangle \right).\] 

It suffices to upper bound $\sum_c \Pr(c) \sum_{t \in \Tl} \left\langle p_{t,c}, \widetilde{\ell}^2_{t,c} \right\rangle .$ We have
\begin{align*}
    &\sum_c \Pr(c) \sum_{t \in \Tl} \left\langle p_{t,c}, \widetilde{\ell}^2_{t,c} \right\rangle \\
    %
    =&\sum_c \Pr(c) \sum_{t \in \Tl} p_{t,c}(a_t) \widetilde{\ell}^2_{t,c}(a_t) \\
    %
    =&\sum_c \Pr(c) \sum_{t \in \Tl} p_{t,c}(a_t) \frac{\ell^2_{t,c}(a_t)}{\left(f_e(a_t) + \gamma\right)^2} \\
    %
    \le& \sum_{t \in \Tl} \sum_{c} \Pr(c) p_{t,c}(a_t) \frac{1}{\left(f_e(a_t) + \gamma\right)^2} \\
    %
    =&  \sum_{t \in \Tl} \frac{p_t(a_t)}{\left(f_e(a_t) + \gamma\right)^2}. 
\end{align*}
Assuming event $G$ holds, we have \[\sum_{t \in \Tl} \frac{p_t(a_t)}{\left(f_e(a_t) + \gamma\right)^2} \le 2 \sum_{t \in \Tl} \frac{1}{f_e(a_t) + \gamma}. \]
%
We then focus on upper bounding $ \sum_{t \in \Tl} \frac{1}{f_e(a_t) + \gamma}.$ 

We have
\begin{itemize}
    \item The sum of conditional expectations $\sum_{t \in \Tl} \E\left[\frac{1}{f_e(a_t) + \gamma} \big| \His_{t-1} \right] \le KT.$
    %
    \item Each term $\frac{1}{f_e(a_t) + \gamma} \le \frac{1}{\gamma}.$
    %
    \item The sum of conditional quadratic expectations
        \begin{align*}
            &\sum_{t \in \Tl} \E\left[ \left(\frac{1}{f_e(a_t) + \gamma}\right)^2 \big| \His_{t-1} \right]\\
            %
            =& \sum_{t \in \Tl} \sum_a \frac{f_e(a)}{\left(f_e(a) + \gamma\right)^2}\\
            %
            \le& \sum_{t \in \Tl} \sum_a \frac{1}{f_e(a) + \gamma}.
        \end{align*}
\end{itemize}

By Freedman's inequality, we have that for any $\lambda \in (0,\gamma]$ and any $\delta \in (0,1)$, the following inequality holds with probability at least $1-\delta$:
\[ \sum_{t \in \Tl} \frac{1}{f_e(a_t) + \gamma} \le \lambda \sum_{t \in \Tl} \sum_a \frac{1}{f_e(a) + \gamma} + \frac{1}{\lambda} \log(\frac{1}{\delta}) + KT. \]
We pick $\lambda = \gamma$ to get that
\[ \sum_{t \in \Tl} \frac{1}{f_e(a_t) + \gamma} \le 2 KT + \frac{1}{\gamma} \log(\frac{1}{\delta}) \]
with probability at least $1-\delta$.

Substituting this inequality back, we get that the folowing inequality holds with probability at least $\Pr(G) - \delta$:
\begin{align*}
    &\sum_{c} \Pr(c) \left( \frac{1}{\eta} \log K  + \frac{\eta}{2} \sum_{t \in \Tl} \left\langle p_{t,c}, \widehat{\ell}^2_{t,c} \right\rangle \right) \\
    %
    \le& \frac{1}{\eta} \log K + 4 \eta  \sum_{t \in \Tl} \frac{1}{f_e(a_t) + \gamma}\\
    %
    \le&  \frac{1}{\eta} \log K + 4 \eta \left( 2 KT + \frac{1}{\gamma} \log(\frac{1}{\delta}) \right).
\end{align*}

\subsubsection{Third}
Here we bound the third term \[ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle. \] 
We decompose it as
\begin{align*}
    &\sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle\\
    %
    =& \sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] \right\rangle \\
    &+ \sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle.
\end{align*}

The first term satisfies 
\begin{align*}
    &\sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] \right\rangle \\
    %
    =&\sum_{t \in \Tl} \sum_c \Pr(c) \sum_{a} p_{t,c}(a) \ell_{t,c}(a)  \frac{\gamma}{f_e(a) + \gamma} \\
    %
    \le& \sum_{t \in \Tl} \sum_{a} p_{t}(a)  \frac{\gamma}{f_e(a) + \gamma}.
\end{align*}
Assuming event $G$ holds, we have
\begin{align*}
    &\sum_{t \in \Tl} \sum_{a} p_{t}(a)  \frac{\gamma}{f_e(a) + \gamma} \\
    %
    \le& 2 \sum_{t \in \Tl} \sum_{a} \gamma \le 2KT\gamma. \\
    %
\end{align*}

We then bound the second term $\sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle.$ 
%
For each time step $t \in \Tl$, we define an indicator function \[L_t \triangleq \indi\left(\forall a, p_{t}(a) \le 4 f_e(a) \right).\] Note that event $G$ implies $\forall t \in \Tel, L_t = 1.$ 
%
Thus we have 
\begin{align*}
    &\sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle \\
    %
    =& \sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle L_t.
\end{align*}
when event $G$ holds. We then assume event $G$ holds and focus on upper bounding \[\sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle L_t.\] 

Since the probability vector $p_{t,c}$ is determined at time $t-1$, the indicator function $L_t$ is also determined at time $t-1$. Thus the summand random variable \[\sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle L_t\] satisfies
\begin{align*}
    &\E\left[ \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle L_t \big| \His_{t-1} \right]\\
    %
    =& \E\left[ \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle \big| \His_{t-1} \right] L_t\\
    %
    =& 0.
\end{align*}
Thus the sequence of random varialbes \[\left\{ \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle L_t \right\}_{t \in \Tl}\] forms a martingale difference sequence with respect to filtration $\{ \His_t \}_{t \in \Tl}$.

The summand random variable further satisfies
\begin{align*}
     & \sum_c \Pr(c) \left\langle p_{t,c},  \widetilde{\ell}_{t,c} \right\rangle L_t \\
     %
     =& \sum_c \Pr(c) p_{t,c}(a_t) \frac{\ell_{t,c}(a_t)}{f_e(a_t) + \gamma} L_t \\
     %
     \le& \sum_c \Pr(c) p_{t,c}(a_t) \frac{1}{f_e(a_t) + \gamma} L_t \\
     %
     =&   \frac{p_t(a_t)}{f_e(a_t) + \gamma} L_t\\
     %
     \le& 4.
\end{align*}

Then by Azuma-Hoeffding inequality, the following inequality holds with probability at least $1- \delta$:
\[\sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle L_t \le 4 \sqrt{T \log(\frac{1}{\delta})}.\]
Thus we have
\[\sum_{t \in \Tl} \sum_c \Pr(c) \left\langle p_{t,c}, \E\left[\widetilde{\ell}_{t,c}\big| \His_{t-1}\right] - \widetilde{\ell}_{t,c} \right\rangle \le  4 \sqrt{T \log(\frac{1}{\delta})}\]
with probability at least $\Pr(G) - \delta$.

Combining the first term and the second term, we get that
\[ \sum_{t \in \Tl}  \sum_{c} \Pr(c) \left\langle p_{t,c}, \ell_{t,c} - \widetilde{\ell}_{t,c} \right\rangle \le 4 \sqrt{T \log(\frac{1}{\delta})} + 2KT\gamma \]
with probability at least $\Pr(G) - \delta$.

\section{Comibined}
Combining \Cref{lemma:used_loss_reduction}, the first, the second, the third, the forth, and the fifth inequality,  we get that the following inequality holds
\begin{align*}
    &\Reg(\pi)\\
    %
    \le&  2 \sqrt{T \log(\frac{1}{\delta})} \\
    &+ 4 \sqrt{T \log(\frac{1}{\delta})} \\
    &+ 2 \frac{1}{\eta} \log K + 8 \eta \left( 2 KT + \frac{1}{\gamma} \log(\frac{1}{\delta}) \right) \\
    &+ 8 \sqrt{T \log(\frac{1}{\delta})} + 4KT\gamma\\
    &+ 8 K \gamma T +  2\frac{K \exp(-\iota) T}{\gamma} + 2\frac{98 K T \iota}{L} + 2\frac{\gamma^2 L K T}{\iota} \\
    &+ 16\left(\sqrt{2KT\iota \log(\frac{\delta}{2})} + 2\sqrt{2\frac{TK^2}{L}\iota \log(\frac{\delta}{2})}\right)\\
    &+  30 \sqrt{T\log(\frac{1}{\delta})}\\
    &+ 2(\frac{8 \cdot 36 \iota}{\gamma} + 2\frac{8}{\gamma}) \log(1/\delta) + 2KT \exp(-\iota)
\end{align*}
with probability at least $\Pr(G) - 8\delta$.

